Alchemical geometry relaxation

We propose to relax geometries throughout chemical compound space (CCS) using alchemical perturbation density functional theory (APDFT). APDFT refers to perturbation theory involving changes in nuclear charges within approximate solutions to Schr\"odinger's equation. We give an analytical formula to calculate the mixed second order energy derivatives with respect to both, nuclear charges and nuclear positions (named "alchemical force"), within the restricted Hartree-Fock case. We have implemented and studied the formula for its use in geometry relaxation of various reference and target molecules. We have also analysed the convergence of the alchemical force perturbation series, as well as basis set effects. Interpolating alchemically predicted energies, forces, and Hessian to a Morse potential yields more accurate geometries and equilibrium energies than when performing a standard Newton Raphson step. Our numerical predictions for small molecules including BF, CO, N2, CH$_4$, NH$_3$, H$_2$O, and HF yield mean absolute errors of of equilibrium energies and bond lengths smaller than 10 mHa and 0.01 Bohr for 4$^\text{th}$ order APDFT predictions, respectively. Our alchemical geometry relaxation still preserves the combinatorial efficiency of APDFT: Based on a single coupled perturbed Hartree Fock derivative for benzene we provide numerical predictions of equilibrium energies and relaxed structures of all the 17 iso-electronic charge-netural BN-doped mutants with averaged absolute deviations of $\sim$27 mHa and $\sim$0.12 Bohr, respectively.

==> 2E_nucnuc.tex <==
\subsection{\label{sec:nucnuc_terms} Nuclear nuclear energy derivatives}
Derivative of the nuclear nuclear electrostatic repulsion can be calculated analytically as the derivative of a classical charge distribution.
The nuclear nuclear interaction energy has a formulation:
\begin{equation} \label{E_nucnuc}
    E_{NN}=\sum_P^{atoms}{\sum_Q^{Q>P} \frac{Z_P Z_Q}{|\mathbf{R}_P-\mathbf{R}_Q |}}
\end{equation}
The alchemical derivatives of the energy are:
\begin{equation} \label{nucnuc_ad}
\begin{aligned}
\frac{\partial E_{NN}}{\partial Z_I}=\sum_Q^{Q\ne I} \frac{Z_Q}{|\mathbf{R}_I-\mathbf{R}_Q|} \\
\frac{\partial^2 E_{NN}}{\partial Z_I\partial Z_J}
=\frac{1-\delta_{IJ}}{|\mathbf{R}_I-\mathbf{R}_J|}
\end{aligned}
\end{equation}

The nuclear nuclear contributions to the alchemical force are:

\begin{equation}
\begin{aligned} \label{nucnuc_af}
\frac{\partial E_{NN}}{\partial x_I}&=
\sum_Q^{Q\ne I} \frac{Z_I Z_Q (x_I-x_Q) }{|\mathbf{R}_I-\mathbf{R}_Q|^3} 
\\
\frac{\partial^2 E_{NN}}{\partial Z_J \partial x_I}&=\left(\sum_Q^{Q\ne I} \frac{Z_Q (x_I-x_Q) }{|\mathbf{R}_I-\mathbf{R}_Q|^3}\ \delta_{IJ}\right)\\
&+\frac{Z_I (x_I-x_J) }{|\mathbf{R}_I-\mathbf{R}_J|^3}(1-\delta_{IJ})
\\
\frac{\partial^3 E_{NN}}{\partial Z_K\partial Z_J \partial x_I}
&=\frac{(x_I-x_K)}{|\mathbf{R_I}-\mathbf{R_K} |^3} (1-\delta_{IK})\delta_{IJ}\\
&+\frac{(x_I-x_J)}{|\mathbf{R_I}-\mathbf{R_J}|^3} (1-\delta_{IJ})\delta_{IK}\\
\end{aligned}
\end{equation}
All the nuclear nuclear terms are zero for alchemical derivatives of order higher than two.
